Few-shot Incremental Event Detection

Event detection tasks can enable the quick detection of events from texts and provide powerful support for downstream natural language processing tasks. Most such methods can only detect a fixed set of predefined event classes. To extend them to detect a new class without losing the ability to detect old classes requires costly retraining of the model from scratch. Incremental learning can effectively solve this problem, but it requires abundant data of new classes. In practice, however, the lack of high-quality labeled data of new event classes makes it difficult to obtain enough data for model training. To address the above mentioned issues, we define a new task, few-shot incremental event detection, which focuses on learning to detect a new event class with limited data, while retaining the ability to detect old classes to the extent possible. We created a benchmark dataset IFSED for the few-shot incremental event detection task based on FewEvent and propose two benchmarks, IFSED-K and IFSED-KP. Experimental results show that our approach has a higher F1-score than baseline methods and is more stable.

==> abstract.tex <==
\begin{abstract}

However, in the real world, new classes are still challenging and labeled data is scarce. Existing methods for learning new event types through large amounts of data have limitations. Therefore, in order to solve the above problem, we define a new task in the domain of event detection, which is few-shot incremental event detection. This task requires the implementation of two parts, namely retaining previous event types and learning new event types in each round with limited samples. We recreated and release a benchmark dataset in the few-shot incremental event detection based on FewEvent. In this new task, the dataset we published is more appropriate than FewEvent dataset. In addition, we propose two benchmark approaches, IFSED-K and IFSED-KP, which can address this new issue in different ways. Experiments have shown that our approach has a higher F1 score and is more stable than baseline.


\end{abstract}
